Towards Precise Prediction Uncertainty in GNNs: Refining GNNs with Topology-grouping Strategy

Recent advancements in graph neural networks (GNNs) have highlighted the critical need of calibrating model predictions, with neighborhood prediction similarity recognized as a pivotal component. Existing studies suggest that nodes with analogous neighborhood prediction similarity often exhibit similar calibration characteristics. Building on this insight, recent approaches incorporate neighborhood similarity into node-wise temperature scaling techniques. However, our analysis reveals that this assumption does not hold universally. Calibration errors can differ significantly even among nodes with comparable neighborhood similarity, depending on their confidence levels. This necessitates a re-evaluation of existing GNN calibration methods, as a single, unified approach may lead to sub-optimal calibration. In response, we introduce **Simi-Mailbox**, a novel approach that categorizes nodes by both neighborhood similarity and their own confidence, irrespective of proximity or connectivity. Our method allows fine-grained calibration by employing *group-specific* temperature scaling, with each temperature tailored to address the specific miscalibration level of affiliated nodes, rather than adhering to a uniform trend based on neighborhood similarity. Extensive experiments demonstrate the effectiveness of our **Simi-Mailbox** across diverse datasets on different GNN architectures, achieving up to 13.79\% error reduction compared to uncalibrated GNN predictions.

==> Table2-1.tex <==
{\renewcommand{\arraystretch}{1.2}
\begin{table*}[t]
    \begin{minipage}{.5\textwidth}
    \caption{Calibration duration (reported in seconds) for our proposed calibration method and baselines on large-scale datasets, averaged over 75 repetitions ($\pm$ STD). A lower value indicates enhanced calibration efficiency.}
    \centering
    \resizebox{\textwidth}{!}{
    \huge{
    % \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{ c | c | c | p }
          \hline
          \textbf{Method} & {CaGCN} & {GATS} & {\textsc{Simi-Mailbox}} \\
          \hline
          \multirow{2}{*}{Arxiv} & GCN & 
          20.84 \fontsize{15}{16}\selectfont$\pm$ 2.69 &
          48.89 \fontsize{15}{16}\selectfont$\pm$ 11.39 &
          \textbf{8.37 \fontsize{15}{16}\selectfont$\pm$ 1.10 (-40.52 sec)}\\
          & SAGE & 
          23.02 \fontsize{15}{16}\selectfont$\pm$ 4.44 &
          61.67 \fontsize{15}{16}\selectfont$\pm$ 16.89 &
          \textbf{4.32 \fontsize{15}{16}\selectfont$\pm$ 0.34 (-57.35 sec)}\\
          \hline
          
          \multirow{4}{*}{Reddit} & GCN &
          55.98 \fontsize{15}{16}\selectfont$\pm$ 13.76 &
          72.90 \fontsize{15}{16}\selectfont$\pm$ 19.98 &
          \textbf{10.59 \fontsize{15}{16}\selectfont$\pm$ 0.51 (-62.31 sec)}\\
          & SAGE & 
          78.13 \fontsize{15}{16}\selectfont$\pm$ 27.35 &
          192.01 \fontsize{15}{16}\selectfont$\pm$ 177.57 &
          \textbf{9.80 \fontsize{15}{16}\selectfont$\pm$ 0.80 (-182.21 sec)}\\
          \hline
    \end{tabular}
    }
    }
    % \end{adjustbox}
    \label{Table2-1}
    \end{minipage}
\end{table*}
}


==> Table4.tex <==
{\renewcommand{\arraystretch}{1.2}
% \begin{table*}[hbt!]
  \begin{table*}[t]
    \caption{Class-wise ECE results (reported in percentage) for our proposed calibration method and baselines, averaged over 75 repetitions ($\pm$ STD). A lower score indicates better calibration performance.}
    % {\LARGE
    \centering
    % \resizebox{.95\textwidth}{!}{
    \resizebox{\textwidth}{!}{
    \huge{
    \begin{tabular}{ c | c | c | c | c | c | c | c | c }
    %{ l | l | l | l | l | l | l | l | l | l | l }
     \hline\hline
     % & {\begin{tabular}[c]{@{}c@{}}LCCal\\ w/CaGCN\end{tabular}}
     % & {\begin{tabular}[c]{@{}c@{}}LCCal\\ w/GATS\end{tabular}}
     \multicolumn{2}{ c |}{\textbf{Methods}} & {{UnCal.}} & {{TS}} & {{VS}} & {{ETS}} & {{CaGCN}} & {{GATS}} & {{LCCal}}\\
     \hline
     % \textbf{Datasets} & \textbf{GNNs} & Hits@20 & Hits@50 & Hits@20 & Hits@50 & Hits@20 & Hits@50 & Hits@20 & Hits@50 & Hits@20 & Hits@50\\
     \hline
     \multirow{2}{*}{Cora} & GCN & 
     {4.23 \fontsize{15}{16}\selectfont$\pm$ 1.21} & 
     {2.05 \fontsize{15}{16}\selectfont$\pm$ 0.24} & 
     {2.10 \fontsize{15}{16}\selectfont$\pm$ 0.29} &  
     {2.06 \fontsize{15}{16}\selectfont$\pm$ 0.23} &  
     {2.21 \fontsize{15}{16}\selectfont$\pm$ 0.30} &  
     %{4.18 \fontsize{15}{16}\selectfont$\pm$ 1.25} & 
     {2.01 \fontsize{15}{16}\selectfont$\pm$ 0.22} &  
     %{3.54 \fontsize{15}{16}\selectfont$\pm$ 1.22} & 
     \textbf{{1.92 \fontsize{15}{16}\selectfont$\pm$ 0.20}}\\
     & GAT & 
     {5.04 \fontsize{15}{16}\selectfont$\pm$ 1.43} & 
     {1.97 \fontsize{15}{16}\selectfont$\pm$ 0.27} &  
     {1.96 \fontsize{15}{16}\selectfont$\pm$ 0.25} &  
     {1.95 \fontsize{15}{16}\selectfont$\pm$ 0.29} &  
     {2.09 \fontsize{15}{16}\selectfont$\pm$ 0.28} &  
     %{4.32 \fontsize{15}{16}\selectfont$\pm$ 1.32} & 
     {2.00 \fontsize{15}{16}\selectfont$\pm$ 0.25} &  
     %{3.74 \fontsize{15}{16}\selectfont$\pm$ 0.94} & 
     \textbf{{1.87 \fontsize{15}{16}\selectfont$\pm$ 0.25}}\\
     \hline
     
     \multirow{2}{*}{Citeseer} & GCN & 
     {5.06 \fontsize{15}{16}\selectfont$\pm$ 2.79} &  
     {2.97 \fontsize{15}{16}\selectfont$\pm$ 0.74} &  
     \textbf{2.78 \fontsize{15}{16}\selectfont$\pm$ 0.45} & 
     {2.95 \fontsize{15}{16}\selectfont$\pm$ 0.76} &  
     {3.34 \fontsize{15}{16}\selectfont$\pm$ 0.77} &  
     %{5.37 \fontsize{15}{16}\selectfont$\pm$ 1.71} & 
     {2.88 \fontsize{15}{16}\selectfont$\pm$ 0.78} & 
     %{4.14 \fontsize{15}{16}\selectfont$\pm$ 1.13} & 
     {2.88 \fontsize{15}{16}\selectfont$\pm$ 1.18}\\
     & GAT & 
     {6.50 \fontsize{15}{16}\selectfont$\pm$ 2.25} & 
     {3.03 \fontsize{15}{16}\selectfont$\pm$ 0.46} & 
     \textbf{2.84 \fontsize{15}{16}\selectfont$\pm$ 0.42} & 
     {3.01 \fontsize{15}{16}\selectfont$\pm$ 0.44} & 
     {3.19 \fontsize{15}{16}\selectfont$\pm$ 0.45} & 
     %{5.05 \fontsize{15}{16}\selectfont$\pm$ 1.54} & 
     {2.96 \fontsize{15}{16}\selectfont$\pm$ 0.43} & 
     %{4.46 \fontsize{15}{16}\selectfont$\pm$ 0.87} & 
     {3.04 \fontsize{15}{16}\selectfont$\pm$ 0.77}\\
     \hline
     
     \multirow{2}{*}{Pubmed} & GCN & 
     {5.09 \fontsize{15}{16}\selectfont$\pm$ 0.96} & 
     {1.38 \fontsize{15}{16}\selectfont$\pm$ 0.27} & 
     {1.52 \fontsize{15}{16}\selectfont$\pm$ 0.29} & 
     {1.39 \fontsize{15}{16}\selectfont$\pm$ 0.26} & 
     {1.35 \fontsize{15}{16}\selectfont$\pm$ 0.33} & 
     %{1.17 \fontsize{15}{16}\selectfont$\pm$ 0.37} & 
     \textbf{1.26 \fontsize{15}{16}\selectfont$\pm$ 0.27} & 
     %{0.99 \fontsize{15}{16}\selectfont$\pm$ 0.26} & 
     {1.35 \fontsize{15}{16}\selectfont$\pm$ 0.28}\\
     & GAT & 
     {7.40 \fontsize{15}{16}\selectfont$\pm$ 1.06} & 
     {1.81 \fontsize{15}{16}\selectfont$\pm$ 0.34} & 
     {1.78 \fontsize{15}{16}\selectfont$\pm$ 0.26} & 
     {1.81 \fontsize{15}{16}\selectfont$\pm$ 0.34} & 
     \textbf{1.70 \fontsize{15}{16}\selectfont$\pm$ 0.36} & 
     %{1.22 \fontsize{15}{16}\selectfont$\pm$ 0.29} & 
     {1.83 \fontsize{15}{16}\selectfont$\pm$ 0.31} & 
     %{1.48 \fontsize{15}{16}\selectfont$\pm$ 0.29} & 
     {1.86 \fontsize{15}{16}\selectfont$\pm$ 0.34}\\
     \hline
    
     \multirow{2}{*}{CoraFull} & GCN & 
     {0.35 \fontsize{15}{16}\selectfont$\pm$ 0.03} & 
     {0.34 \fontsize{15}{16}\selectfont$\pm$ 0.02} & 
     {0.34 \fontsize{15}{16}\selectfont$\pm$ 0.01} & 
     {0.34 \fontsize{15}{16}\selectfont$\pm$ 0.02} & 
     {0.33 \fontsize{15}{16}\selectfont$\pm$ 0.04} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     {0.33 \fontsize{15}{16}\selectfont$\pm$ 0.02} & 
     %{2.43 \fontsize{15}{16}\selectfont$\pm$ 0.51} & 
     \textbf{{0.32 \fontsize{15}{16}\selectfont$\pm$ 0.01}}\\
     & GAT & 
     {0.33 \fontsize{15}{16}\selectfont$\pm$ 0.03} & 
     {0.32 \fontsize{15}{16}\selectfont$\pm$ 0.01} & 
     {0.32 \fontsize{15}{16}\selectfont$\pm$ 0.01} & 
     {0.32 \fontsize{15}{16}\selectfont$\pm$ 0.01} & 
     {0.36 \fontsize{15}{16}\selectfont$\pm$ 0.08} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     \textbf{{0.31 \fontsize{15}{16}\selectfont$\pm$ 0.02}} &  
     %{2.42 \fontsize{15}{16}\selectfont$\pm$ 0.45} & 
     \textbf{{0.31 \fontsize{15}{16}\selectfont$\pm$ 0.02}}\\
     \hline
     
     \multirow{2}{*}{Computers} & GCN & 
     {0.95 \fontsize{15}{16}\selectfont$\pm$ 0.14} & 
     {0.92 \fontsize{15}{16}\selectfont$\pm$ 0.10} & 
     {0.91 \fontsize{15}{16}\selectfont$\pm$ 0.13} & 
     {0.94 \fontsize{15}{16}\selectfont$\pm$ 0.11} & 
     {0.83 \fontsize{15}{16}\selectfont$\pm$ 0.09} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     {0.89 \fontsize{15}{16}\selectfont$\pm$ 0.07} & 
     %{1.7 \fontsize{15}{16}\selectfont$\pm$ 0.45} & 
     \textbf{{0.82 \fontsize{15}{16}\selectfont$\pm$ 0.10}}\\
     & GAT & 
     {0.82 \fontsize{15}{16}\selectfont$\pm$ 0.13} & 
     {0.80 \fontsize{15}{16}\selectfont$\pm$ 0.10} & 
     \textbf{0.78 \fontsize{15}{16}\selectfont$\pm$ 0.11} & 
     {0.81 \fontsize{15}{16}\selectfont$\pm$ 0.10} & 
     {0.80 \fontsize{15}{16}\selectfont$\pm$ 0.10} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     \textbf{0.78 \fontsize{15}{16}\selectfont$\pm$ 0.09} &  
     %{1.15 \fontsize{15}{16}\selectfont$\pm$ 0.41} & 
     {0.80 \fontsize{15}{16}\selectfont$\pm$ 0.11}\\
     \hline

     \multirow{2}{*}{Photo} & GCN & 
     {0.86 \fontsize{15}{16}\selectfont$\pm$ 0.21} & 
     {0.78 \fontsize{15}{16}\selectfont$\pm$ 0.14} & 
     {0.81 \fontsize{15}{16}\selectfont$\pm$ 0.15} & 
     {0.78 \fontsize{15}{16}\selectfont$\pm$ 0.15} & 
     {0.80 \fontsize{15}{16}\selectfont$\pm$ 0.08} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     {0.76 \fontsize{15}{16}\selectfont$\pm$ 0.11} & 
     %{1.2 \fontsize{15}{16}\selectfont$\pm$ 0.4} & 
     \textbf{{0.73 \fontsize{15}{16}\selectfont$\pm$ 0.07}}\\
     & GAT & 
     {0.99 \fontsize{15}{16}\selectfont$\pm$ 0.33} & 
     {0.86 \fontsize{15}{16}\selectfont$\pm$ 0.16} & 
     {0.83 \fontsize{15}{16}\selectfont$\pm$ 0.17} & 
     {0.86 \fontsize{15}{16}\selectfont$\pm$ 0.17} & 
     {0.86 \fontsize{15}{16}\selectfont$\pm$ 0.13} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     {0.85 \fontsize{15}{16}\selectfont$\pm$ 0.17} & 
     %{1.39 \fontsize{15}{16}\selectfont$\pm$ 0.55} & 
     \textbf{0.82 \fontsize{15}{16}\selectfont$\pm$ 0.13}\\
     \hline

     \multirow{2}{*}{CS} & GCN & 
     {0.40 \fontsize{15}{16}\selectfont$\pm$ 0.15} & 
     {0.30 \fontsize{15}{16}\selectfont$\pm$ 0.03} & 
     {0.32 \fontsize{15}{16}\selectfont$\pm$ 0.03} & 
     \textbf{0.29 \fontsize{15}{16}\selectfont$\pm$ 0.03} & 
     {0.42 \fontsize{15}{16}\selectfont$\pm$ 0.10} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     \textbf{0.29 \fontsize{15}{16}\selectfont$\pm$ 0.03} &
     %{0.76 \fontsize{15}{16}\selectfont$\pm$ 0.22} & 
     {0.31 \fontsize{15}{16}\selectfont$\pm$ 0.04}\\
     & GAT & 
     {0.38 \fontsize{15}{16}\selectfont$\pm$ 0.15} & 
     {0.34 \fontsize{15}{16}\selectfont$\pm$ 0.04} & 
     {0.34 \fontsize{15}{16}\selectfont$\pm$ 0.03} & 
     \textbf{0.33 \fontsize{15}{16}\selectfont$\pm$ 0.04} & 
     {0.43 \fontsize{15}{16}\selectfont$\pm$ 0.09} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     \textbf{0.33 \fontsize{15}{16}\selectfont$\pm$ 0.04} & 
     %{0.97 \fontsize{15}{16}\selectfont$\pm$ 0.31} & 
     {0.34 \fontsize{15}{16}\selectfont$\pm$ 0.05}\\
     \hline

     \multirow{2}{*}{Physics} & GCN & 
     {0.41 \fontsize{15}{16}\selectfont$\pm$ 0.12} & 
     {0.36 \fontsize{15}{16}\selectfont$\pm$ 0.06} & 
     \textbf{0.34 \fontsize{15}{16}\selectfont$\pm$ 0.04} & 
     {0.36 \fontsize{15}{16}\selectfont$\pm$ 0.06} & 
     {0.46 \fontsize{15}{16}\selectfont$\pm$ 0.14} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     {0.36 \fontsize{15}{16}\selectfont$\pm$ 0.05} & 
     %{0.43 \fontsize{15}{16}\selectfont$\pm$ 0.15} & 
     {0.37 \fontsize{15}{16}\selectfont$\pm$ 0.09}\\
     & GAT & 
     {0.39 \fontsize{15}{16}\selectfont$\pm$ 0.07} & 
     {0.39 \fontsize{15}{16}\selectfont$\pm$ 0.07} & 
     \textbf{0.37 \fontsize{15}{16}\selectfont$\pm$ 0.06} & 
     {0.39 \fontsize{15}{16}\selectfont$\pm$ 0.06} & 
     {0.52 \fontsize{15}{16}\selectfont$\pm$ 0.14} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     {0.38 \fontsize{15}{16}\selectfont$\pm$ 0.06} & 
     %{0.51 \fontsize{15}{16}\selectfont$\pm$ 0.15} & 
     {0.40 \fontsize{15}{16}\selectfont$\pm$ 0.09}\\
     \hline
    \hline\hline
    \end{tabular}}}
    \label{Table4}
  \end{table*}
}


==> Table5.tex <==
{\renewcommand{\arraystretch}{1.2}
% \begin{table*}[hbt!]
  \begin{table*}[t]
    \caption{Brier Score results for our proposed calibration method and baselines, averaged over 75 repetitions ($\pm$ STD). A lower score indicates better calibration performance.}
    % {\LARGE
    \centering
    % \resizebox{.95\textwidth}{!}{
    \resizebox{\textwidth}{!}{
    \Huge{
    \begin{tabular}{ c | c | c | c | c | c | c | c | c }
    %{ l | l | l | l | l | l | l | l | l | l | l }
     \hline\hline
     % & {\begin{tabular}[c]{@{}c@{}}LCCal\\ w/CaGCN\end{tabular}}
     % & {\begin{tabular}[c]{@{}c@{}}LCCal\\ w/GATS\end{tabular}}
     \multicolumn{2}{ c |}{\textbf{Methods}} & {{UnCal.}} & {{TS}} & {{VS}} & {{ETS}} & {{CaGCN}} & {{GATS}} & {{LCCal}}\\
     \hline
     % \textbf{Datasets} & \textbf{GNNs} & Hits@20 & Hits@50 & Hits@20 & Hits@50 & Hits@20 & Hits@50 & Hits@20 & Hits@50 & Hits@20 & Hits@50\\
     \hline
     \multirow{2}{*}{Cora} & GCN &  
     {0.2844 \fontsize{15}{16}\selectfont$\pm$ 0.0202} &  
     {0.2556 \fontsize{15}{16}\selectfont$\pm$ 0.0095} &  
     {0.2564 \fontsize{15}{16}\selectfont$\pm$ 0.0103} &  
     {0.2556 \fontsize{15}{16}\selectfont$\pm$ 0.0095} &  
     {0.2612 \fontsize{15}{16}\selectfont$\pm$ 0.0109} &  
     %{4.18 \fontsize{15}{16}\selectfont$\pm$ 1.25} & 
     {0.2554 \fontsize{15}{16}\selectfont$\pm$ 0.0102} &  
     %{3.54 \fontsize{15}{16}\selectfont$\pm$ 1.22} & 
     \textbf{0.2530 \fontsize{15}{16}\selectfont$\pm$ 0.0098} \\
     & GAT & 
     {0.2820 \fontsize{15}{16}\selectfont$\pm$ 0.0285} & 
     {0.2422 \fontsize{15}{16}\selectfont$\pm$ 0.0090} &  
     {0.2421 \fontsize{15}{16}\selectfont$\pm$ 0.0106} &  
     {0.2421 \fontsize{15}{16}\selectfont$\pm$ 0.0090} &  
     {0.2470 \fontsize{15}{16}\selectfont$\pm$ 0.0093} &  
     %{4.32 \fontsize{15}{16}\selectfont$\pm$ 1.32} & 
     {0.2428 \fontsize{15}{16}\selectfont$\pm$ 0.0086} &  
     %{3.74 \fontsize{15}{16}\selectfont$\pm$ 0.94} & 
     \textbf{0.2413 \fontsize{15}{16}\selectfont$\pm$ 0.0090}\\
     \hline
     
     \multirow{2}{*}{Citeseer} & GCN & 
     {0.4372 \fontsize{15}{16}\selectfont$\pm$ 0.0511} &  
     {0.4098 \fontsize{15}{16}\selectfont$\pm$ 0.0110} &  
     {0.4103 \fontsize{15}{16}\selectfont$\pm$ 0.0096} &  
     {0.4097 \fontsize{15}{16}\selectfont$\pm$ 0.0112} &  
     {0.4182 \fontsize{15}{16}\selectfont$\pm$ 0.0136} &  
     %{5.37 \fontsize{15}{16}\selectfont$\pm$ 1.71} & 
     \textbf{0.4087 \fontsize{15}{16}\selectfont$\pm$ 0.0111} & 
     %{4.14 \fontsize{15}{16}\selectfont$\pm$ 1.13} & 
     {0.4100 \fontsize{15}{16}\selectfont$\pm$ 0.0149}\\
     & GAT & 
     {0.4513 \fontsize{15}{16}\selectfont$\pm$ 0.0424} & 
     {0.4095 \fontsize{15}{16}\selectfont$\pm$ 0.0090} & 
     {0.4098 \fontsize{15}{16}\selectfont$\pm$ 0.0099} & 
     {0.4093 \fontsize{15}{16}\selectfont$\pm$ 0.0088} & 
     {0.4145 \fontsize{15}{16}\selectfont$\pm$ 0.0101} & 
     %{5.05 \fontsize{15}{16}\selectfont$\pm$ 1.54} & 
     \textbf{0.4089 \fontsize{15}{16}\selectfont$\pm$ 0.0085} & 
     %{4.46 \fontsize{15}{16}\selectfont$\pm$ 0.87} & 
     {0.4091 \fontsize{15}{16}\selectfont$\pm$ 0.0105}\\
     \hline
     
     \multirow{2}{*}{Pubmed} & GCN & 
     {0.2138 \fontsize{15}{16}\selectfont$\pm$ 0.0069} & 
     {0.2022 \fontsize{15}{16}\selectfont$\pm$ 0.0035} & 
     {0.2025 \fontsize{15}{16}\selectfont$\pm$ 0.0036} & 
     {0.3662 \fontsize{15}{16}\selectfont$\pm$ 0.0064} & 
     {0.2005 \fontsize{15}{16}\selectfont$\pm$ 0.0037} & 
     %{1.17 \fontsize{15}{16}\selectfont$\pm$ 0.37} & 
     \textbf{0.2019 \fontsize{15}{16}\selectfont$\pm$ 0.0035} & 
     %{0.99 \fontsize{15}{16}\selectfont$\pm$ 0.26} & 
     {0.2028 \fontsize{15}{16}\selectfont$\pm$ 0.0035}\\
     & GAT & 
     {0.2394 \fontsize{15}{16}\selectfont$\pm$ 0.0090} & 
     {0.2189 \fontsize{15}{16}\selectfont$\pm$ 0.0039} & 
     \textbf{0.2185 \fontsize{15}{16}\selectfont$\pm$ 0.0039} & 
     {0.2189 \fontsize{15}{16}\selectfont$\pm$ 0.0039} & 
     {0.3858 \fontsize{15}{16}\selectfont$\pm$ 0.0070} & 
     {0.2188 \fontsize{15}{16}\selectfont$\pm$ 0.0039} & 
     %{1.22 \fontsize{15}{16}\selectfont$\pm$ 0.29} & 
     %{1.48 \fontsize{15}{16}\selectfont$\pm$ 0.29} & 
     {0.2192 \fontsize{15}{16}\selectfont$\pm$ 0.0042}\\
     \hline
    
     \multirow{2}{*}{CoraFull} & GCN & 
     {0.5224 \fontsize{15}{16}\selectfont$\pm$ 0.0065} & 
     {0.5206 \fontsize{15}{16}\selectfont$\pm$ 0.0049} & 
     {0.5199 \fontsize{15}{16}\selectfont$\pm$ 0.0048} & 
     {0.5206 \fontsize{15}{16}\selectfont$\pm$ 0.0049} & 
     {0.5208 \fontsize{15}{16}\selectfont$\pm$ 0.0122} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     \textbf{0.5156 \fontsize{15}{16}\selectfont$\pm$ 0.0048} & 
     %{2.43 \fontsize{15}{16}\selectfont$\pm$ 0.51} & 
     {0.5198 \fontsize{15}{16}\selectfont$\pm$ 0.0052}\\
     & GAT & 
     {0.5116 \fontsize{15}{16}\selectfont$\pm$ 0.0073} & 
     {0.5098 \fontsize{15}{16}\selectfont$\pm$ 0.0058} & 
     \textbf{0.5082 \fontsize{15}{16}\selectfont$\pm$ 0.0056} & 
     {0.5098 \fontsize{15}{16}\selectfont$\pm$ 0.0058} & 
     {0.5196 \fontsize{15}{16}\selectfont$\pm$ 0.0179} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     {0.5088 \fontsize{15}{16}\selectfont$\pm$ 0.0058} &  
     %{2.42 \fontsize{15}{16}\selectfont$\pm$ 0.45} & 
     {0.5084 \fontsize{15}{16}\selectfont$\pm$ 0.0059}\\
     \hline
     
     \multirow{2}{*}{Computers} & GCN & 
     {0.1855 \fontsize{15}{16}\selectfont$\pm$ 0.0069} & 
     {0.1849 \fontsize{15}{16}\selectfont$\pm$ 0.0062} & 
     {0.1843 \fontsize{15}{16}\selectfont$\pm$ 0.0062} & 
     {0.1850 \fontsize{15}{16}\selectfont$\pm$ 0.0062} & 
     \textbf{0.1811 \fontsize{15}{16}\selectfont$\pm$ 0.0062} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     {0.1840 \fontsize{15}{16}\selectfont$\pm$ 0.0058} & 
     %{1.7 \fontsize{15}{16}\selectfont$\pm$ 0.45} & 
     {0.1813 \fontsize{15}{16}\selectfont$\pm$ 0.0077}\\
     & GAT & 
     {0.1731 \fontsize{15}{16}\selectfont$\pm$ 0.0079} & 
     {0.1729 \fontsize{15}{16}\selectfont$\pm$ 0.0076} & 
     \textbf{0.1713 \fontsize{15}{16}\selectfont$\pm$ 0.0067} & 
     {0.1729 \fontsize{15}{16}\selectfont$\pm$ 0.0076} & 
     {0.1734 \fontsize{15}{16}\selectfont$\pm$ 0.0074} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     {0.1729 \fontsize{15}{16}\selectfont$\pm$ 0.0075} &  
     %{1.15 \fontsize{15}{16}\selectfont$\pm$ 0.41} & 
     {0.1715 \fontsize{15}{16}\selectfont$\pm$ 0.0073}\\
     \hline

     \multirow{2}{*}{Photo} & GCN & 
     {0.1166 \fontsize{15}{16}\selectfont$\pm$ 0.0062} & 
     {0.1156 \fontsize{15}{16}\selectfont$\pm$ 0.0057} & 
     {0.2913 \fontsize{15}{16}\selectfont$\pm$ 0.0122} & 
     {0.2728 \fontsize{15}{16}\selectfont$\pm$ 0.0132} & 
     {0.1164 \fontsize{15}{16}\selectfont$\pm$ 0.0051} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     {0.1151 \fontsize{15}{16}\selectfont$\pm$ 0.0054} & 
     %{1.2 \fontsize{15}{16}\selectfont$\pm$ 0.4} & 
     \textbf{{0.1148 \fontsize{15}{16}\selectfont$\pm$ 0.0050}}\\
     & GAT & 
     {0.1173 \fontsize{15}{16}\selectfont$\pm$ 0.0103} & 
     {0.1161 \fontsize{15}{16}\selectfont$\pm$ 0.0085} & 
     \textbf{0.1144 \fontsize{15}{16}\selectfont$\pm$ 0.0078} & 
     {0.1161 \fontsize{15}{16}\selectfont$\pm$ 0.0085} & 
     {0.1167 \fontsize{15}{16}\selectfont$\pm$ 0.0080} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     {0.1161 \fontsize{15}{16}\selectfont$\pm$ 0.0084} & 
     %{1.39 \fontsize{15}{16}\selectfont$\pm$ 0.55} & 
     {0.1160 \fontsize{15}{16}\selectfont$\pm$ 0.0079}\\
     \hline

     \multirow{2}{*}{CS} & GCN & 
     {0.1064 \fontsize{15}{16}\selectfont$\pm$ 0.0043} & 
     {0.1018 \fontsize{15}{16}\selectfont$\pm$ 0.0023} & 
     {0.1020 \fontsize{15}{16}\selectfont$\pm$ 0.0020} & 
     {0.1018 \fontsize{15}{16}\selectfont$\pm$ 0.0023} & 
     {0.1064 \fontsize{15}{16}\selectfont$\pm$ 0.0043} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     \textbf{0.1016 \fontsize{15}{16}\selectfont$\pm$ 0.0024} & 
     %{0.76 \fontsize{15}{16}\selectfont$\pm$ 0.22} & 
     {0.1018 \fontsize{15}{16}\selectfont$\pm$ 0.0025}\\
     & GAT & 
     {0.1131 \fontsize{15}{16}\selectfont$\pm$ 0.0051} & 
     {0.1123 \fontsize{15}{16}\selectfont$\pm$ 0.0028} & 
     \textbf{0.1120 \fontsize{15}{16}\selectfont$\pm$ 0.0023} & 
     {0.1123 \fontsize{15}{16}\selectfont$\pm$ 0.0028} & 
     {0.1149 \fontsize{15}{16}\selectfont$\pm$ 0.0035} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     {0.1123 \fontsize{15}{16}\selectfont$\pm$ 0.0027} & 
     %{0.97 \fontsize{15}{16}\selectfont$\pm$ 0.31} & 
     {0.1131 \fontsize{15}{16}\selectfont$\pm$ 0.0023}\\
     \hline

     \multirow{2}{*}{Physics} & GCN & 
     {0.0614 \fontsize{15}{16}\selectfont$\pm$ 0.0020} & 
     {0.0614 \fontsize{15}{16}\selectfont$\pm$ 0.0019} & 
     {0.0614 \fontsize{15}{16}\selectfont$\pm$ 0.0018} & 
     {0.0614 \fontsize{15}{16}\selectfont$\pm$ 0.0019} & 
     {0.0625 \fontsize{15}{16}\selectfont$\pm$ 0.0021} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     \textbf{0.0613 \fontsize{15}{16}\selectfont$\pm$ 0.0019} & 
     %{0.43 \fontsize{15}{16}\selectfont$\pm$ 0.15} & 
     {0.0616 \fontsize{15}{16}\selectfont$\pm$ 0.0019}\\
     & GAT & 
     {0.0658 \fontsize{15}{16}\selectfont$\pm$ 0.0017} & 
     {0.0658 \fontsize{15}{16}\selectfont$\pm$ 0.0017} & 
     \textbf{0.0657 \fontsize{15}{16}\selectfont$\pm$ 0.0017} & 
     {0.0658 \fontsize{15}{16}\selectfont$\pm$ 0.0017} & 
     {0.0666 \fontsize{15}{16}\selectfont$\pm$ 0.0018} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     \textbf{0.0657 \fontsize{15}{16}\selectfont$\pm$ 0.0017} & 
     %{0.51 \fontsize{15}{16}\selectfont$\pm$ 0.15} & 
     {0.0660 \fontsize{15}{16}\selectfont$\pm$ 0.0017}\\
     \hline
    \hline\hline
    \end{tabular}}}
    \label{Table5}
  \end{table*}
}


==> Table6.tex <==
{\renewcommand{\arraystretch}{1.2}
% \begin{table*}[hbt!]
  \begin{table*}[t]
    \caption{KDE-ECE results (reported in percentage) for our proposed calibration method and baselines, averaged over 75 repetitions ($\pm$ STD). A lower score indicates better calibration performance.}
    % {\LARGE
    \centering
    % \resizebox{.95\textwidth}{!}{
    \resizebox{\textwidth}{!}{
    \huge{
    \begin{tabular}{ c | c | c | c | c | c | c | c | c }
    %{ l | l | l | l | l | l | l | l | l | l | l }
     \hline\hline
     % & {\begin{tabular}[c]{@{}c@{}}LCCal\\ w/CaGCN\end{tabular}}
     % & {\begin{tabular}[c]{@{}c@{}}LCCal\\ w/GATS\end{tabular}}
     \multicolumn{2}{ c |}{\textbf{Methods}} & {{UnCal.}} & {{TS}} & {{VS}} & {{ETS}} & {{CaGCN}} & {{GATS}} & {{LCCal}}\\
     \hline
     % \textbf{Datasets} & \textbf{GNNs} & Hits@20 & Hits@50 & Hits@20 & Hits@50 & Hits@20 & Hits@50 & Hits@20 & Hits@50 & Hits@20 & Hits@50\\
     \hline
     \multirow{2}{*}{Cora} & GCN & 
     {13.08 \fontsize{15}{16}\selectfont$\pm$ 4.47} &
     {3.22 \fontsize{15}{16}\selectfont$\pm$ 1.14} &
     {3.58 \fontsize{15}{16}\selectfont$\pm$ 1.26} &  
     {3.27 \fontsize{15}{16}\selectfont$\pm$ 1.14} &  
     {4.20 \fontsize{15}{16}\selectfont$\pm$ 1.42} &  
     %{4.18 \fontsize{15}{16}\selectfont$\pm$ 1.25} & 
     {3.03 \fontsize{15}{16}\selectfont$\pm$ 1.26} &  
     %{3.54 \fontsize{15}{16}\selectfont$\pm$ 1.22} & 
     \textbf{2.79 \fontsize{15}{16}\selectfont$\pm$ 0.83} \\
     & GAT & 
     {15.87 \fontsize{15}{16}\selectfont$\pm$ 4.99} & 
     {2.74 \fontsize{15}{16}\selectfont$\pm$ 0.78} &  
     {2.86 \fontsize{15}{16}\selectfont$\pm$ 0.88} &  
     {2.74 \fontsize{15}{16}\selectfont$\pm$ 0.77} &  
     {3.40 \fontsize{15}{16}\selectfont$\pm$ 1.18} &  
     %{4.32 \fontsize{15}{16}\selectfont$\pm$ 1.32} & 
     {2.95 \fontsize{15}{16}\selectfont$\pm$ 1.09} &  
     %{3.74 \fontsize{15}{16}\selectfont$\pm$ 0.94} & 
     \textbf{2.33 \fontsize{15}{16}\selectfont$\pm$ 0.48} \\
     \hline
     
     \multirow{2}{*}{Citeseer} & GCN & 
     {12.31 \fontsize{15}{16}\selectfont$\pm$ 8.49} &  
     {4.85 \fontsize{15}{16}\selectfont$\pm$ 1.58} &  
     {4.71 \fontsize{15}{16}\selectfont$\pm$ 1.47} &  
     {4.81 \fontsize{15}{16}\selectfont$\pm$ 1.58} &  
     {6.37 \fontsize{15}{16}\selectfont$\pm$ 1.55} &  
     %{5.37 \fontsize{15}{16}\selectfont$\pm$ 1.71} & 
     {4.26 \fontsize{15}{16}\selectfont$\pm$ 1.58} & 
     %{4.14 \fontsize{15}{16}\selectfont$\pm$ 1.13} & 
     \textbf{4.06 \fontsize{15}{16}\selectfont$\pm$ 2.54}\\
     & GAT & 
     {17.05 \fontsize{15}{16}\selectfont$\pm$ 7.12} & 
     {4.70 \fontsize{15}{16}\selectfont$\pm$ 1.36} & 
     {4.24 \fontsize{15}{16}\selectfont$\pm$ 1.43} & 
     {4.59 \fontsize{15}{16}\selectfont$\pm$ 1.35} & 
     {5.66 \fontsize{15}{16}\selectfont$\pm$ 1.21} & 
     %{5.05 \fontsize{15}{16}\selectfont$\pm$ 1.54} & 
     {4.00 \fontsize{15}{16}\selectfont$\pm$ 1.28} & 
     %{4.46 \fontsize{15}{16}\selectfont$\pm$ 0.87} & 
     \textbf{{3.59 \fontsize{15}{16}\selectfont$\pm$ 2.04}}\\
     \hline
     
     \multirow{2}{*}{Pubmed} & GCN & 
     {7.52 \fontsize{15}{16}\selectfont$\pm$ 1.40} & 
     {1.33 \fontsize{15}{16}\selectfont$\pm$ 0.29} & 
     {1.59 \fontsize{15}{16}\selectfont$\pm$ 0.39} & 
     {1.37 \fontsize{15}{16}\selectfont$\pm$ 0.31} & 
     {1.26 \fontsize{15}{16}\selectfont$\pm$ 0.39} & 
     %{1.17 \fontsize{15}{16}\selectfont$\pm$ 0.37} & 
     \textbf{1.06 \fontsize{15}{16}\selectfont$\pm$ 0.26} & 
     %{0.99 \fontsize{15}{16}\selectfont$\pm$ 0.26} & 
     {1.27 \fontsize{15}{16}\selectfont$\pm$ 0.28}\\
     & GAT & 
     {10.62 \fontsize{15}{16}\selectfont$\pm$ 1.73} & 
     {1.15 \fontsize{15}{16}\selectfont$\pm$ 0.35} & 
     {1.14 \fontsize{15}{16}\selectfont$\pm$ 0.28} & 
     {1.15 \fontsize{15}{16}\selectfont$\pm$ 0.34} & 
     \textbf{1.07 \fontsize{15}{16}\selectfont$\pm$ 0.27} & 
     %{1.22 \fontsize{15}{16}\selectfont$\pm$ 0.29} & 
     {1.10 \fontsize{15}{16}\selectfont$\pm$ 0.28} & 
     %{1.48 \fontsize{15}{16}\selectfont$\pm$ 0.29} & 
     {1.31 \fontsize{15}{16}\selectfont$\pm$ 0.35}\\
     \hline
    
     \multirow{2}{*}{CoraFull} & GCN & 
     {6.30 \fontsize{15}{16}\selectfont$\pm$ 1.14} & 
     {5.52 \fontsize{15}{16}\selectfont$\pm$ 0.49} & 
     {5.69 \fontsize{15}{16}\selectfont$\pm$ 0.51} & 
     {5.49 \fontsize{15}{16}\selectfont$\pm$ 0.51} & 
     {5.57 \fontsize{15}{16}\selectfont$\pm$ 2.32} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     {3.66 \fontsize{15}{16}\selectfont$\pm$ 0.67} & 
     %{2.43 \fontsize{15}{16}\selectfont$\pm$ 0.51} & 
     \textbf{{2.13 \fontsize{15}{16}\selectfont$\pm$ 0.57}}\\
     & GAT & 
     {5.28 \fontsize{15}{16}\selectfont$\pm$ 1.36} & 
     {4.36 \fontsize{15}{16}\selectfont$\pm$ 0.50} & 
     {4.38 \fontsize{15}{16}\selectfont$\pm$ 0.50} & 
     {4.33 \fontsize{15}{16}\selectfont$\pm$ 0.50} & 
     {7.00 \fontsize{15}{16}\selectfont$\pm$ 4.03} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     {3.48 \fontsize{15}{16}\selectfont$\pm$ 0.47} &  
     %{2.42 \fontsize{15}{16}\selectfont$\pm$ 0.45} & 
     \textbf{{1.95 \fontsize{15}{16}\selectfont$\pm$ 0.59}}\\
     \hline
     
     \multirow{2}{*}{Computers} & GCN & 
     {3.00 \fontsize{15}{16}\selectfont$\pm$ 0.81} & 
     {2.64 \fontsize{15}{16}\selectfont$\pm$ 0.64} & 
     {2.74 \fontsize{15}{16}\selectfont$\pm$ 0.69} & 
     {2.75 \fontsize{15}{16}\selectfont$\pm$ 0.69} & 
     {1.61 \fontsize{15}{16}\selectfont$\pm$ 0.41} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     {2.14 \fontsize{15}{16}\selectfont$\pm$ 0.61} & 
     %{1.7 \fontsize{15}{16}\selectfont$\pm$ 0.45} & 
     \textbf{{1.41 \fontsize{15}{16}\selectfont$\pm$ 0.30}}\\
     & GAT & 
     {1.78 \fontsize{15}{16}\selectfont$\pm$ 0.83} & 
     {1.60 \fontsize{15}{16}\selectfont$\pm$ 0.63} & 
     {1.65 \fontsize{15}{16}\selectfont$\pm$ 0.60} & 
     {1.67 \fontsize{15}{16}\selectfont$\pm$ 0.69} & 
     {1.70 \fontsize{15}{16}\selectfont$\pm$ 0.50} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     \textbf{1.48 \fontsize{15}{16}\selectfont$\pm$ 0.54} &  
     %{1.15 \fontsize{15}{16}\selectfont$\pm$ 0.41} & 
     {1.56 \fontsize{15}{16}\selectfont$\pm$ 0.57}\\
     \hline

     \multirow{2}{*}{Photo} & GCN & 
     {2.45 \fontsize{15}{16}\selectfont$\pm$ 1.23} & 
     {1.81 \fontsize{15}{16}\selectfont$\pm$ 0.92} & 
     {1.95 \fontsize{15}{16}\selectfont$\pm$ 0.95} & 
     {1.87 \fontsize{15}{16}\selectfont$\pm$ 0.96} & 
     {1.66 \fontsize{15}{16}\selectfont$\pm$ 0.41} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     {1.65 \fontsize{15}{16}\selectfont$\pm$ 0.68} & 
     %{1.2 \fontsize{15}{16}\selectfont$\pm$ 0.4} & 
     \textbf{{1.50 \fontsize{15}{16}\selectfont$\pm$ 0.34}}\\
     & GAT & 
     {2.50 \fontsize{15}{16}\selectfont$\pm$ 1.49} & 
     {1.71 \fontsize{15}{16}\selectfont$\pm$ 0.72} & 
     {1.82 \fontsize{15}{16}\selectfont$\pm$ 0.86} & 
     {1.79 \fontsize{15}{16}\selectfont$\pm$ 0.77} & 
     {1.68 \fontsize{15}{16}\selectfont$\pm$ 0.56} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     {1.72 \fontsize{15}{16}\selectfont$\pm$ 0.66} & 
     %{1.39 \fontsize{15}{16}\selectfont$\pm$ 0.55} & 
     \textbf{1.61 \fontsize{15}{16}\selectfont$\pm$ 0.49}\\
     \hline

     \multirow{2}{*}{CS} & GCN & 
     {2.19 \fontsize{15}{16}\selectfont$\pm$ 1.33} & 
     {1.12 \fontsize{15}{16}\selectfont$\pm$ 0.10} & 
     {1.12 \fontsize{15}{16}\selectfont$\pm$ 0.18} & 
     {1.12 \fontsize{15}{16}\selectfont$\pm$ 0.10} & 
     {1.94 \fontsize{15}{16}\selectfont$\pm$ 0.92} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     \textbf{1.08 \fontsize{15}{16}\selectfont$\pm$ 0.12} & 
     %{0.76 \fontsize{15}{16}\selectfont$\pm$ 0.22} & 
     {1.25 \fontsize{15}{16}\selectfont$\pm$ 0.30}\\
     & GAT & 
     {1.61 \fontsize{15}{16}\selectfont$\pm$ 1.24} & 
     {1.09 \fontsize{15}{16}\selectfont$\pm$ 0.17} & 
     {1.10 \fontsize{15}{16}\selectfont$\pm$ 0.21} & 
     {1.09 \fontsize{15}{16}\selectfont$\pm$ 0.17} & 
     {1.89 \fontsize{15}{16}\selectfont$\pm$ 0.88} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     \textbf{1.07 \fontsize{15}{16}\selectfont$\pm$ 0.13} & 
     %{0.97 \fontsize{15}{16}\selectfont$\pm$ 0.31} & 
     {1.13 \fontsize{15}{16}\selectfont$\pm$ 0.32}\\
     \hline

     \multirow{2}{*}{Physics} & GCN & 
     {0.97 \fontsize{15}{16}\selectfont$\pm$ 0.30} & 
     {0.83 \fontsize{15}{16}\selectfont$\pm$ 0.09} & 
     \textbf{0.82 \fontsize{15}{16}\selectfont$\pm$ 0.07} & 
     {0.83 \fontsize{15}{16}\selectfont$\pm$ 0.09} & 
     {0.93 \fontsize{15}{16}\selectfont$\pm$ 0.19} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     {0.85 \fontsize{15}{16}\selectfont$\pm$ 0.09} & 
     %{0.43 \fontsize{15}{16}\selectfont$\pm$ 0.15} & 
     {0.90 \fontsize{15}{16}\selectfont$\pm$ 0.19}\\
     & GAT & 
     {0.85 \fontsize{15}{16}\selectfont$\pm$ 0.12} & 
     {0.83 \fontsize{15}{16}\selectfont$\pm$ 0.10} & 
     {0.84 \fontsize{15}{16}\selectfont$\pm$ 0.10} & 
     {0.83 \fontsize{15}{16}\selectfont$\pm$ 0.10} & 
     {1.04 \fontsize{15}{16}\selectfont$\pm$ 0.23} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     \textbf{0.82 \fontsize{15}{16}\selectfont$\pm$ 0.08} & 
     %{0.51 \fontsize{15}{16}\selectfont$\pm$ 0.15} & 
     {0.90 \fontsize{15}{16}\selectfont$\pm$ 0.19}\\
     \hline
    \hline\hline
    \end{tabular}}}
    \label{Table6}
  \end{table*}
}


==> Table7.tex <==
{\renewcommand{\arraystretch}{1.2}
% \begin{table*}[hbt!]
  \begin{table*}[h!]
    \caption{NLL results for our proposed calibration method and baselines, averaged over 75 repetitions ($\pm$ STD). A lower score indicates better calibration performance.}
    % {\LARGE
    \centering
    % \resizebox{.95\textwidth}{!}{
    \resizebox{\textwidth}{!}{
    \Huge{
    \begin{tabular}{ c | c | c | c | c | c | c | c | c }
    %{ l | l | l | l | l | l | l | l | l | l | l }
     \hline\hline
     % & {\begin{tabular}[c]{@{}c@{}}LCCal\\ w/CaGCN\end{tabular}}
     % & {\begin{tabular}[c]{@{}c@{}}LCCal\\ w/GATS\end{tabular}}
     \multicolumn{2}{ c |}{\textbf{Methods}} & {{UnCal.}} & {{TS}} & {{VS}} & {{ETS}} & {{CaGCN}} & {{GATS}} & {{LCCal}}\\
     \hline
     % \textbf{Datasets} & \textbf{GNNs} & Hits@20 & Hits@50 & Hits@20 & Hits@50 & Hits@20 & Hits@50 & Hits@20 & Hits@50 & Hits@20 & Hits@50\\
     \hline
     \multirow{2}{*}{Cora} & GCN & 
     {0.6235 \fontsize{15}{16}\selectfont$\pm$ 0.0463} & 
     {0.5622 \fontsize{15}{16}\selectfont$\pm$ 0.0306} & 
     {0.5753 \fontsize{15}{16}\selectfont$\pm$ 0.0404} &  
     {0.5604 \fontsize{15}{16}\selectfont$\pm$ 0.0304} &  
     {0.6691 \fontsize{15}{16}\selectfont$\pm$ 0.0799} &  
     %{4.18 \fontsize{15}{16}\selectfont$\pm$ 1.25} & 
     {0.5573 \fontsize{15}{16}\selectfont$\pm$ 0.0296} &  
     %{3.54 \fontsize{15}{16}\selectfont$\pm$ 1.22} & 
     \textbf{{0.5435 \fontsize{15}{16}\selectfont$\pm$ 0.0287}}\\
     & GAT & 
     {0.6211 \fontsize{15}{16}\selectfont$\pm$ 0.0632} & 
     {0.5187 \fontsize{15}{16}\selectfont$\pm$ 0.0252} &  
     {0.5246 \fontsize{15}{16}\selectfont$\pm$ 0.0339} &  
     {0.5173 \fontsize{15}{16}\selectfont$\pm$ 0.0246} &  
     {0.5884 \fontsize{15}{16}\selectfont$\pm$ 0.0683} &  
     %{4.32 \fontsize{15}{16}\selectfont$\pm$ 1.32} & 
     {0.5207 \fontsize{15}{16}\selectfont$\pm$ 0.0250} &  
     %{3.74 \fontsize{15}{16}\selectfont$\pm$ 0.94} & 
     \textbf{{0.5062 \fontsize{15}{16}\selectfont$\pm$ 0.0208}}\\
     \hline
     
     \multirow{2}{*}{Citeseer} & GCN & 
     {0.9255 \fontsize{15}{16}\selectfont$\pm$ 0.1067} &  
     {0.8809 \fontsize{15}{16}\selectfont$\pm$ 0.0504} &  
     {0.8732 \fontsize{15}{16}\selectfont$\pm$ 0.0247} &  
     {0.8778 \fontsize{15}{16}\selectfont$\pm$ 0.0411} &  
     {0.9395 \fontsize{15}{16}\selectfont$\pm$ 0.0589} &  
     %{5.37 \fontsize{15}{16}\selectfont$\pm$ 1.71} & 
     {0.8735 \fontsize{15}{16}\selectfont$\pm$ 0.0506} & 
     %{4.14 \fontsize{15}{16}\selectfont$\pm$ 1.13} & 
     \textbf{{0.8706 \fontsize{15}{16}\selectfont$\pm$ 0.0469}}\\
     & GAT & 
     {0.9599 \fontsize{15}{16}\selectfont$\pm$ 0.0859} & 
     {0.8739 \fontsize{15}{16}\selectfont$\pm$ 0.0303} & 
     {0.8694 \fontsize{15}{16}\selectfont$\pm$ 0.0224} & 
     {0.8723 \fontsize{15}{16}\selectfont$\pm$ 0.0276} & 
     {0.9092 \fontsize{15}{16}\selectfont$\pm$ 0.0404} & 
     %{5.05 \fontsize{15}{16}\selectfont$\pm$ 1.54} & 
     {0.8698 \fontsize{15}{16}\selectfont$\pm$ 0.0277} & 
     %{4.46 \fontsize{15}{16}\selectfont$\pm$ 0.87} & 
     \textbf{{0.8662 \fontsize{15}{16}\selectfont$\pm$ 0.0268}}\\
     \hline
     
     \multirow{2}{*}{Pubmed} & GCN & 
     {0.3947 \fontsize{15}{16}\selectfont$\pm$ 0.0140} & 
     {0.3678 \fontsize{15}{16}\selectfont$\pm$ 0.0064} & 
     {0.3681 \fontsize{15}{16}\selectfont$\pm$ 0.0064} & 
     {0.3662 \fontsize{15}{16}\selectfont$\pm$ 0.0065} & 
     \textbf{0.3589 \fontsize{15}{16}\selectfont$\pm$ 0.0083} & 
     %{1.17 \fontsize{15}{16}\selectfont$\pm$ 0.37} & 
     {0.3641 \fontsize{15}{16}\selectfont$\pm$ 0.0058} & 
     %{0.99 \fontsize{15}{16}\selectfont$\pm$ 0.26} & 
     {0.3656 \fontsize{15}{16}\selectfont$\pm$ 0.0061}\\
     & GAT & 
     {0.4417 \fontsize{15}{16}\selectfont$\pm$ 0.0178} & 
     {0.3884 \fontsize{15}{16}\selectfont$\pm$ 0.0073} & 
     {0.3877 \fontsize{15}{16}\selectfont$\pm$ 0.0068} & 
     {0.3884 \fontsize{15}{16}\selectfont$\pm$ 0.0073} & 
     \textbf{0.3858 \fontsize{15}{16}\selectfont$\pm$ 0.0070} & 
     %{1.22 \fontsize{15}{16}\selectfont$\pm$ 0.29} & 
     {0.3879 \fontsize{15}{16}\selectfont$\pm$ 0.0070} & 
     %{1.48 \fontsize{15}{16}\selectfont$\pm$ 0.29} & 
     {0.3886 \fontsize{15}{16}\selectfont$\pm$ 0.0075}\\
     \hline
    
     \multirow{2}{*}{CoraFull} & GCN & 
     {1.4288 \fontsize{15}{16}\selectfont$\pm$ 0.0197} & 
     {1.4262 \fontsize{15}{16}\selectfont$\pm$ 0.0172} & 
     {1.4277 \fontsize{15}{16}\selectfont$\pm$ 0.0193} & 
     {1.4204 \fontsize{15}{16}\selectfont$\pm$ 0.0174} & 
     {1.4626 \fontsize{15}{16}\selectfont$\pm$ 0.1453} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     \textbf{1.3991 \fontsize{15}{16}\selectfont$\pm$ 0.0169} & 
     %{2.43 \fontsize{15}{16}\selectfont$\pm$ 0.51} & 
     {1.4110 \fontsize{15}{16}\selectfont$\pm$ 0.0157}\\
     & GAT & 
     {1.3666 \fontsize{15}{16}\selectfont$\pm$ 0.0222} & 
     {1.3625 \fontsize{15}{16}\selectfont$\pm$ 0.0178} & 
     {1.3643 \fontsize{15}{16}\selectfont$\pm$ 0.0176} & 
     {1.3612 \fontsize{15}{16}\selectfont$\pm$ 0.0175} & 
     {1.4708 \fontsize{15}{16}\selectfont$\pm$ 0.2100} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     {1.3546 \fontsize{15}{16}\selectfont$\pm$ 0.0173} &  
     %{2.42 \fontsize{15}{16}\selectfont$\pm$ 0.45} & 
     \textbf{{1.3500 \fontsize{15}{16}\selectfont$\pm$ 0.0168}}\\
     \hline
     
     \multirow{2}{*}{Computers} & GCN & 
     {0.4292 \fontsize{15}{16}\selectfont$\pm$ 0.0099} & 
     {0.4291 \fontsize{15}{16}\selectfont$\pm$ 0.0098} & 
     {0.4290 \fontsize{15}{16}\selectfont$\pm$ 0.0100} & 
     {0.4123 \fontsize{15}{16}\selectfont$\pm$ 0.0129} & 
     {0.4310 \fontsize{15}{16}\selectfont$\pm$ 0.0344} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     {0.4242 \fontsize{15}{16}\selectfont$\pm$ 0.0117} & 
     %{1.7 \fontsize{15}{16}\selectfont$\pm$ 0.45} & 
     \textbf{{0.4069 \fontsize{15}{16}\selectfont$\pm$ 0.0095}}\\
     & GAT & 
     {0.3768 \fontsize{15}{16}\selectfont$\pm$ 0.0157} & 
     {0.3765 \fontsize{15}{16}\selectfont$\pm$ 0.0153} & 
     {0.3758 \fontsize{15}{16}\selectfont$\pm$ 0.0151} & 
     \textbf{0.3721 \fontsize{15}{16}\selectfont$\pm$ 0.0159} & 
     {0.4022 \fontsize{15}{16}\selectfont$\pm$ 0.0360} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     {0.3765 \fontsize{15}{16}\selectfont$\pm$ 0.0157} &  
     %{1.15 \fontsize{15}{16}\selectfont$\pm$ 0.41} & 
     {0.3737 \fontsize{15}{16}\selectfont$\pm$ 0.0155}\\
     \hline

     \multirow{2}{*}{Photo} & GCN & 
     {0.2877 \fontsize{15}{16}\selectfont$\pm$ 0.0108} & 
     {0.2892 \fontsize{15}{16}\selectfont$\pm$ 0.0110} & 
     {0.2913 \fontsize{15}{16}\selectfont$\pm$ 0.0122} & 
     \textbf{0.2723 \fontsize{15}{16}\selectfont$\pm$ 0.0132} & 
     {0.3799 \fontsize{15}{16}\selectfont$\pm$ 0.0830} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     {0.2867 \fontsize{15}{16}\selectfont$\pm$ 0.0113} & 
     %{1.2 \fontsize{15}{16}\selectfont$\pm$ 0.4} & 
     {0.2892 \fontsize{15}{16}\selectfont$\pm$ 0.0110}\\
     & GAT & 
     {0.2722 \fontsize{15}{16}\selectfont$\pm$ 0.0208} & 
     {0.2717 \fontsize{15}{16}\selectfont$\pm$ 0.0176} & 
     {0.2709 \fontsize{15}{16}\selectfont$\pm$ 0.0174} & 
     \textbf{0.2674 \fontsize{15}{16}\selectfont$\pm$ 0.0195} & 
     {0.3213 \fontsize{15}{16}\selectfont$\pm$ 0.0525} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     {0.2714 \fontsize{15}{16}\selectfont$\pm$ 0.0176} & 
     %{1.39 \fontsize{15}{16}\selectfont$\pm$ 0.55} & 
     {0.2763 \fontsize{15}{16}\selectfont$\pm$ 0.0163}\\
     \hline

     \multirow{2}{*}{CS} & GCN & 
     {0.2196 \fontsize{15}{16}\selectfont$\pm$ 0.0119} & 
     {0.2142 \fontsize{15}{16}\selectfont$\pm$ 0.0056} & 
     {0.2162 \fontsize{15}{16}\selectfont$\pm$ 0.0049} & 
     {0.2141 \fontsize{15}{16}\selectfont$\pm$ 0.0055} & 
     {0.2760 \fontsize{15}{16}\selectfont$\pm$ 0.0578} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     \textbf{0.2132 \fontsize{15}{16}\selectfont$\pm$ 0.0057} & 
     %{0.76 \fontsize{15}{16}\selectfont$\pm$ 0.22} & 
     \textbf{0.2132 \fontsize{15}{16}\selectfont$\pm$ 0.0061}\\
     & GAT & 
     {0.2443 \fontsize{15}{16}\selectfont$\pm$ 0.0133} & 
     {0.2425 \fontsize{15}{16}\selectfont$\pm$ 0.0065} & 
     {0.2421 \fontsize{15}{16}\selectfont$\pm$ 0.0054} & 
     {0.2421 \fontsize{15}{16}\selectfont$\pm$ 0.0064} & 
     {0.2768 \fontsize{15}{16}\selectfont$\pm$ 0.0304} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     \textbf{0.2416 \fontsize{15}{16}\selectfont$\pm$ 0.0062} & 
     %{0.97 \fontsize{15}{16}\selectfont$\pm$ 0.31} & 
     {0.2433 \fontsize{15}{16}\selectfont$\pm$ 0.0050}\\
     \hline

     \multirow{2}{*}{Physics} & GCN & 
     {0.1199 \fontsize{15}{16}\selectfont$\pm$ 0.0043} & 
     {0.1190 \fontsize{15}{16}\selectfont$\pm$ 0.0035} & 
     {0.1190 \fontsize{15}{16}\selectfont$\pm$ 0.0033} & 
     {0.1190 \fontsize{15}{16}\selectfont$\pm$ 0.0035} & 
     {0.1293 \fontsize{15}{16}\selectfont$\pm$ 0.0116} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     \textbf{0.1188 \fontsize{15}{16}\selectfont$\pm$ 0.0033} & 
     %{0.43 \fontsize{15}{16}\selectfont$\pm$ 0.15} & 
     {0.1198 \fontsize{15}{16}\selectfont$\pm$ 0.0038}\\
     & GAT & 
     {0.1288 \fontsize{15}{16}\selectfont$\pm$ 0.0042} & 
     {0.1287 \fontsize{15}{16}\selectfont$\pm$ 0.0041} & 
     \textbf{0.1284 \fontsize{15}{16}\selectfont$\pm$ 0.0039} & 
     {0.1287 \fontsize{15}{16}\selectfont$\pm$ 0.0041} & 
     {0.1339 \fontsize{15}{16}\selectfont$\pm$ 0.0068} & 
     %{3.62 \fontsize{15}{16}\selectfont$\pm$ 1.9} & 
     {0.1286 \fontsize{15}{16}\selectfont$\pm$ 0.0040} & 
     %{0.51 \fontsize{15}{16}\selectfont$\pm$ 0.15} & 
     {0.1299 \fontsize{15}{16}\selectfont$\pm$ 0.0041}\\
     \hline
    \hline\hline
    \end{tabular}}}
    \label{Table7}
  \end{table*}
}


==> Table_grouping.tex <==
{\renewcommand{\arraystretch}{1.2}
% \begin{table*}[hbt!]
  \begin{table*}[t]
    \caption{Variance of calibration errors ($\mathbf{\times 100}$) involving neighborhood similarity sub-intervals (Neig. Sim.), confidence intervals (Conf), and total nodes (Node-wise).}
    % {\LARGE
    \centering
    % \resizebox{.95\textwidth}{!}{
    \resizebox{\textwidth}{!}{
    {
    \begin{tabular}{ c | c | c | c | c | c | c | c | c | c }
    %{ l | l | l | l | l | l | l | l | l | l | l }
     \hline\hline
     % & {\begin{tabular}[c]{@{}c@{}}LCCal\\ w/CaGCN\end{tabular}}
     % & {\begin{tabular}[c]{@{}c@{}}LCCal\\ w/GATS\end{tabular}}
     \multicolumn{2}{ c |}{\textbf{GNNs}} & {{Cora}} & {{Citeseer}} & {{Pubmed}} & {{Computers}} & {{Photo}} & {{CS}} & {{Physics}} & {{CoraFull}}\\
     \hline
     % \textbf{Datasets} & \textbf{GNNs} & Hits@20 & Hits@50 & Hits@20 & Hits@50 & Hits@20 & Hits@50 & Hits@20 & Hits@50 & Hits@20 & Hits@50\\
     \hline
     \multirow{3}{*}{GCN} & {Node-wise}
     & {6.139} 
     & {1.957}
     & {1.370} 
     & {40.370} 
     & {7.200}
     & {31.470} 
     & {3.312}
     & {34.560}\\
     & {Conf.}
     & {0.065} 
     & {0.060}
     & {0.068} 
     & \textbf{0.060} 
     & {0.052} 
     & {0.058}
     & {0.041} 
     & {0.064} \\
     & \rowcolor{blanchedalmond}{Neig. Sim.}
     & \textbf{0.057} 
     & \textbf{0.046}
     & \textbf{0.061} 
     & {0.062} 
     & \textbf{0.047} 
     & \textbf{0.052}
     & \textbf{0.040} 
     & \textbf{0.057} \\
     \hline
     
     \multirow{3}{*}{GAT} & {Node-wise}
     & {8.656} 
     & {2.570}
     & {1.614} 
     & {44.980} 
     & {14.550} 
     & {42.660}
     & {3.346} 
     & {58.67} \\
     & {Conf.}
     & {0.068} 
     & {0.062}
     & {0.068} 
     & {0.048} 
     & {0.053} 
     & {0.050}
     & \textbf{0.035} 
     & {0.062} \\
     & \rowcolor{blanchedalmond}{Neig. Sim.}
     & \textbf{0.056} 
     & \textbf{0.044}
     & \textbf{0.055} 
     & \textbf{0.045} 
     & \textbf{0.047} 
     & \textbf{0.044}
     & \textbf{0.035} 
     & \textbf{0.055} \\
     % \hline
    \hline\hline
    \end{tabular}}}
    \label{Table_grouping}
    \vskip -5pt
  \end{table*}
}


==> Table_pce1.tex <==
{\renewcommand{\arraystretch}{1.2}
% \begin{table*}[hbt!]
\begin{table*}[t]
\caption{\blue{ECE results (reported in percentage) for our proposed calibration method, GATS and GC without the holdout set. A lower ECE indicates better calibration performance. The best and second best performances are represented by bold and underline texts, respectively.}}
\centering
% \resizebox{.95\textwidth}{!}{
% \scalebox{0.7}{
\resizebox{\textwidth}{!}{
\Huge
{
\begin{tabular}
% {p{1.2cm}|p{0.5cm}p{0.5cm}|p{0.5cm}p{0.5cm}|p{0.5cm}p{0.5cm}|p{0.5cm}p{0.5cm}|p{0.5cm}p{0.5cm}|p{0.5cm}p{0.5cm}|p{0.5cm}p{0.5cm}|p{0.5cm}p{0.5cm}}
{ c | c | c | c | c | c | c | c | c | c }
%{ l | l | l | l | l | l | l | l | l | l | l }
\hline\hline

\multicolumn{2}{ c |}{\textbf{Datasets}} & {Cora} & {Citeseer} & {Pubmed} & {Computers} & {Photo} & {CS} & {Physics} &{CoraFull} \\

\hline
% \textbf{GNNs} & GCN & GAT & GCN & GAT & GCN & GAT & GCN & GAT & GCN & GAT & GCN & GAT & GCN & GAT & GCN & GAT\\
% \hline

\multirow{4}{*}{GCN} 
& GC+TS w/o HO &
{{7.48 \fontsize{15}{20}\selectfont$\pm$ 4.19}} &
{{8.12 \fontsize{15}{20}\selectfont$\pm$ 6.59}} &
{{1.63 \fontsize{15}{20}\selectfont$\pm$ 0.50}} &
{{2.58 \fontsize{15}{20}\selectfont$\pm$ 0.73}} &
{{2.02 \fontsize{15}{20}\selectfont$\pm$ 0.71}} &
{{1.09 \fontsize{15}{20}\selectfont$\pm$ 0.56}} &
\underline{{0.45\fontsize{15}{20}\selectfont$\pm$ 0.18}} &
{{6.02 \fontsize{15}{20}\selectfont$\pm$ 0.98}} \\

& GC+ETS w/o HO &
{{7.09 \fontsize{15}{20}\selectfont$\pm$ 4.15}} &
{{8.22 \fontsize{15}{20}\selectfont$\pm$ 6.58}} &
{{1.65 \fontsize{15}{20}\selectfont$\pm$ 0.46}} &
\underline{{1.61 \fontsize{15}{20}\selectfont$\pm$ 0.50}} &
{{2.19 \fontsize{15}{20}\selectfont$\pm$ 1.35}} &
{{1.13 \fontsize{15}{20}\selectfont$\pm$ 0.60}} &
{{0.56 \fontsize{15}{20}\selectfont$\pm$ 0.24}} &
{{5.60 \fontsize{15}{20}\selectfont$\pm$ 1.14}} \\

& GATS & 
\underline{3.59 \fontsize{15}{20}\selectfont$\pm$ 1.23} &
\underline{4.53 \fontsize{15}{20}\selectfont$\pm$ 1.54} &
\underline{1.01 \fontsize{15}{20}\selectfont$\pm$ 0.33} &
{2.17 \fontsize{15}{20}\selectfont$\pm$ 0.54} &
\underline{1.47 \fontsize{15}{20}\selectfont$\pm$ 0.50} &
\underline{0.92 \fontsize{15}{20}\selectfont$\pm$ 0.30} &
{0.46 \fontsize{15}{20}\selectfont$\pm$ 0.15} &
\underline{3.86 \fontsize{15}{20}\selectfont$\pm$ 0.86} \\

& \rowcolor{blanchedalmond}{\textbf{Ours}} &
\textbf{{2.06 \fontsize{15}{20}\selectfont$\pm$ 0.44}} &
\textbf{{2.76 \fontsize{15}{20}\selectfont$\pm$ 0.56}} &
\textbf{{0.77 \fontsize{15}{20}\selectfont$\pm$ 0.15}} &
\textbf{{1.06 \fontsize{15}{20}\selectfont$\pm$ 0.26}} &
\textbf{{1.04 \fontsize{15}{20}\selectfont$\pm$ 0.35}} &
\textbf{{0.60 \fontsize{15}{20}\selectfont$\pm$ 0.19}} &
\textbf{{0.29 \fontsize{15}{20}\selectfont$\pm$ 0.11}} &
\textbf{{3.47 \fontsize{15}{20}\selectfont$\pm$ 1.32}} \\
\hline

\multirow{4}{*}{GAT} 
& GC+TS w/o HO &
{{7.43 \fontsize{15}{20}\selectfont$\pm$ 5.12}} &
{{6.39 \fontsize{15}{20}\selectfont$\pm$ 5.53}} &
{{1.05 \fontsize{15}{20}\selectfont$\pm$ 0.42}} &
{{1.66 \fontsize{15}{20}\selectfont$\pm$ 0.53}} &
{{1.71 \fontsize{15}{20}\selectfont$\pm$ 0.65}} &
{{1.10 \fontsize{15}{20}\selectfont$\pm$ 0.67}} &
\textbf{{0.42 \fontsize{15}{20}\selectfont$\pm$ 0.16}} &
{{4.49 \fontsize{15}{20}\selectfont$\pm$ 0.70}} \\

& GC+ETS w/o HO &
{{7.22 \fontsize{15}{20}\selectfont$\pm$ 4.97}} &
{{6.57 \fontsize{15}{20}\selectfont$\pm$ 5.61}} &
{{1.25 \fontsize{15}{20}\selectfont$\pm$ 0.57}} &
{{1.56 \fontsize{15}{20}\selectfont$\pm$ 0.52}} &
\underline{{1.50 \fontsize{15}{20}\selectfont$\pm$ 0.74}} &
{{1.14 \fontsize{15}{20}\selectfont$\pm$ 0.77}} &
{{0.57 \fontsize{15}{20}\selectfont$\pm$ 0.24}} &
{{4.03 \fontsize{15}{20}\selectfont$\pm$ 0.81}} \\

& GATS & 
\underline{3.23 \fontsize{15}{20}\selectfont$\pm$ 1.07} &
\underline{4.08 \fontsize{15}{20}\selectfont$\pm$ 1.41} &
\underline{1.02 \fontsize{15}{20}\selectfont$\pm$ 0.38}&
\underline{1.39 \fontsize{15}{20}\selectfont$\pm$ 0.34} &
{1.52 \fontsize{15}{20}\selectfont$\pm$ 0.63} &
\underline{0.88 \fontsize{15}{20}\selectfont$\pm$ 0.22} &
\underline{{0.44 \fontsize{15}{20}\selectfont$\pm$ 0.16}} &
\underline{3.50 \fontsize{15}{20}\selectfont$\pm$ 0.45}\\

& \rowcolor{blanchedalmond}{\textbf{Ours}} & 
\textbf{{2.15 \fontsize{15}{20}\selectfont$\pm$ 0.44}} &
\textbf{{2.97 \fontsize{15}{20}\selectfont$\pm$ 0.58}} &
\textbf{0.73 \fontsize{15}{20}\selectfont$\pm$ 0.17} &
\textbf{{0.98 \fontsize{15}{20}\selectfont$\pm$ 0.38}} &
\textbf{{1.00 \fontsize{15}{20}\selectfont$\pm$ 0.52}} &
\textbf{{0.75 \fontsize{15}{20}\selectfont$\pm$ 0.43}} &
{0.49 \fontsize{15}{20}\selectfont$\pm$ 0.21} &
\textbf{{2.66 \fontsize{15}{20}\selectfont$\pm$ 1.01}}\\
\hline\hline
\end{tabular}}
}
\label{Table_pce1}

\end{table*}
}

==> Table_st_gat.tex <==
{\renewcommand{\arraystretch}{1}
% \begin{table*}[hbt!]
\begin{table*}[t]
\caption{\blue{Average node classification accuracy of various label rate (L/C) for our proposed calibration method and baselines on GAT.}}
\centering
% \resizebox{.95\textwidth}{!}{
% \scalebox{0.7}{
\resizebox{0.8\textwidth}{!}{
\footnotesize
{
\begin{tabular}
{ c c | c | c | a }
\hline\hline

{Datasets} & {L/C} & {UnCal.} & {CaGCN} & {Ours}  \\

\hline

\multirow{3}{*}{Cora} & 20 & 
{ \fontsize{5}{6}\selectfont$\pm$ } &
{ \fontsize{5}{6}\selectfont$\pm$ } &
{ \fontsize{5}{6}\selectfont$\pm$ } \\

& 40 &
{ \fontsize{5}{6}\selectfont$\pm$ } &
{ \fontsize{5}{6}\selectfont$\pm$ } &
{ \fontsize{5}{6}\selectfont$\pm$ } \\

& 60 &
{ \fontsize{5}{6}\selectfont$\pm$ } &
{ \fontsize{5}{6}\selectfont$\pm$ } &
{ \fontsize{5}{6}\selectfont$\pm$ } \\
\hline

\multirow{3}{*}{Citeseer} & 20 & 
{ \fontsize{5}{6}\selectfont$\pm$ } &
{ \fontsize{5}{6}\selectfont$\pm$ } &
{ \fontsize{5}{6}\selectfont$\pm$ } \\

& 40 &
{ \fontsize{5}{6}\selectfont$\pm$ } &
{ \fontsize{5}{6}\selectfont$\pm$ } &
{ \fontsize{5}{6}\selectfont$\pm$ } \\

& 60 &
{ \fontsize{5}{6}\selectfont$\pm$ } &
{ \fontsize{5}{6}\selectfont$\pm$ } &
{ \fontsize{5}{6}\selectfont$\pm$ } \\
\hline

\multirow{3}{*}{Pubmed} & 20 & 
{ \fontsize{5}{6}\selectfont$\pm$ } &
{ \fontsize{5}{6}\selectfont$\pm$ } &
{ \fontsize{5}{6}\selectfont$\pm$ } \\

& 40 &
{ \fontsize{5}{6}\selectfont$\pm$ } &
{ \fontsize{5}{6}\selectfont$\pm$ } &
{ \fontsize{5}{6}\selectfont$\pm$ } \\

& 60 &
{ \fontsize{5}{6}\selectfont$\pm$ } &
{ \fontsize{5}{6}\selectfont$\pm$ } &
{ \fontsize{5}{6}\selectfont$\pm$ } \\

\hline\hline
\end{tabular}}
}
\label{Table_st_gat}

\end{table*}
}

==> hyperparam_sensitivity.tex <==
\begin{wrapfigure}{l}{0.52\textwidth}
\includegraphics[width=1.\linewidth]{hyperparameter_sensitivity.pdf} 
\caption{Hyperparameter sensitivity.}
\label{fig: hyperparam_sensitivity}
% \vskip -8pt
\end{wrapfigure}

==> table_gin.tex <==
{\renewcommand{\arraystretch}{1.}
\begin{table*}[t]
\centering
\caption{\blue{ECE results (reported in percentage) for our proposed calibration method and baselines on GIN, averaged over 75 runs.}}
\resizebox{.95\textwidth}{!}{
\begin{tabular}{ c | c | c | c | c | c | c | c | c }
\hline\hline
\textbf{GIN} & Cora & Citeseer & Pubmed & Computers & Photo & CS & Physics & CoraFull \\ \hline
UnCal. & 11.82 $\pm$ 5.41 & 13.90 $\pm$ 5.02 & 7.16 $\pm$ 2.91 & 8.16 $\pm$ 3.54 & 6.18 $\pm$ 6.59 & 7.23 $\pm$ 2.06 & 4.79 $\pm$ 2.22 & 19.74 $\pm$ 1.09 \\
GATS & 8.34 $\pm$ 2.17 & 10.25 $\pm$ 2.67 & 4.47 $\pm$ 1.86 & 5.73 $\pm$ 2.36 & 3.85 $\pm$ 2.72 & 6.93 $\pm$ 1.59 & 3.55 $\pm$ 1.11 & 17.88 $\pm$ 1.60 \\
\rowcolor{lightgray}\textbf{Ours} & \textbf{6.09 $\pm$ 2.00}
& \textbf{6.91 $\pm$ 2.80}
& \textbf{1.70 $\pm$ 0.43}
& \textbf{1.50 $\pm$ 0.62}
& \textbf{1.55 $\pm$ 1.61}
& \textbf{3.18 $\pm$ 0.93}
& \textbf{1.18 $\pm$ 0.42}
& \textbf{8.23 $\pm$ 4.52} \\ \hline\hline
\end{tabular}}
\label{table_gin}
\end{table*}}

